Spectral atlas of A-type supergiants

Based on high-spectral-resolution observations (R=60000) performed with the 6-m BTA telescope in combination with the echelle spectrograph NES, we have studied the optical spectra of three A-type supergiants: a peculiar supergiant 3 Pup, a post-AGB star BD+48 1220, and a massive $\alpha$ Cyg, which belong to essentially different stages of evolution. A spectral atlas for these stars is prepared in the wavelength interval of 3920 to 6720 \AA.

==> longtab.tex <==

\begin{longtable}{l llc@{\quad} @{\quad}l @{\quad}l @{\quad}l@{\quad}}
\caption{Отождествление линий, их остаточные интенсивности
              и лучевые скорости ${\rm V_r }$\,, км/сек в спектре
	      Cyg\,OB2 - ${\rm \No}$\,12. В скобках указан номер мультиплета
	      }      
\\ \hline
\endfirsthead
\hline
\multicolumn{6}{l}{Табл.\,1, продолжение} \\ \hline
\endhead
\hline
\multicolumn{6}{r}{продолжение на след. странице} \\ \hline
\endfoot
\hline
\endlastfoot
\hline
 Е & & ${\rm \lambda_{lab}}$ &  W$_{\lambda}$, \AA & r  & ${\rm V_r }$  \\
\hline

\hline
\end{longtable}	       			     
\label{lines}

